A Static Pruning Study on Sparse Neural Retrievers

Sparse neural retrievers, such as DeepImpact, uniCOIL and SPLADE, have been introduced recently as an efficient and effective way to perform retrieval with inverted indexes. They aim to learn term importance and, in some cases, document expansions, to provide a more effective document ranking compared to traditional bag-of-words retrieval models such as BM25. However, these sparse neural retrievers have been shown to increase the computational costs and latency of query processing compared to their classical counterparts. To mitigate this, we apply a well-known family of techniques for boosting the efficiency of query processing over inverted indexes: static pruning. We experiment with three static pruning strategies, namely document-centric, term-centric and agnostic pruning, and we assess, over diverse datasets, that these techniques still work with sparse neural retrievers. In particular, static pruning achieves $2\times$ speedup with negligible effectiveness loss ($\leq 2\%$ drop) and, depending on the use case, even $4\times$ speedup with minimal impact on the effectiveness ($\leq 8\%$ drop). Moreover, we show that neural rerankers are robust to candidates from statically pruned indexes.

==> equations.tex <==
\input{preamble.tex}
\begin{document}

\title{For testing equations}

\begin{itemize}
    \item $x_{i,j}$ Output of splade for document $i$ and word $j$
    \item $||B||$ Size of the batch
    \item $||V||$ Size of the vocabulary
\end{itemize}

\section{Carlos}

Thinking of going from FLOPS to an error MSE based on a desired number of activations per dim.

Currently we consider a probability of activation for each dimension. To do so we first compute $p_j = \sum_i \left ( \frac{x_{i,j}}{B} \right)^2$ and then sum it over all dimensions. This gives us the expected flops (as we sum the probability of activation for all dimensions), but it has two problems:

\begin{enumerate}
    \item Considers that the ideal distribution is 0 activations (i.e. nothing activated). While this is normally solved by having a secondary function, this is not ideal as it can cause the network to simply learn a ``dumb'' solution
    \item Very hard to control, especially when ||B|| or ||V|| increases
\end{enumerate}

What we could do is introduce a desired activation probability $\hat{p}$ and then compute the error (MSE for the start) between the estimated probability $p_j$ and the desired one:

\begin{equation}
    \mathcal{L} = \frac{\sum_j||\hat{p}^2 - p_j||_2}{||V||}
\end{equation}

And then to compute the $\hat{p}$ we could simply use $\frac{k}{||V||}$ where $k$ is the desired document size.

$Possible=VN$

$Desired=kN$

$\frac{Desired}{Possible}$

\section{Stephane}
Let $p_i$ be the probability of observing word i in the collection. For instance we could set $p_i=\frac{10^k}{N}$ where $k$ is parameter.

Now in a batch, we estimate $\hat{p_i}=q_i= \sum \frac{s_i}{B(s_i + \tau)}$  and then minimize
the KL between $p_i$ and $q_i$
$$
- p_i \log( q_i) - (1-p_i) \log( 1- q_i)
$$

Penalize by the Flops directly (no proba)of
$$
C_i = \sum_d x_{d,i}/(\tau+ x_{d,i})
$$
the maximum length of the posting list in the batch. 
We can divide by the Batch size to make it normalized

DFR Like measure or Bose Einstein:
$$
- \frac{C_i}{B} \log (p_i)
$$


Maximize Entropy in the Batch? between terms
Orthogonality between terms?

Minimize Entropy on documents
\end{document}

==> tikz/compare_msmarco/mrr/figure.tex <==
\begin{figure}[ht]
     \centering
     \begin{subfigure}[t]{0.7\columnwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{tikz/compare_msmarco/mrr/pisa.tex}
         }
     \end{subfigure}
     \begin{subfigure}[t]{0.29\columnwidth}
         \centering
\adjustbox{max width=\textwidth}{%
         \raisebox{50px}{%
         \input{tikz/compare_msmarco/mrr/legend.tex}}
}
     \end{subfigure}
      \caption{Speedup vs Relative MRR@10 comparison.}
     \label{fig:rq2}
\end{figure}





==> tikz/compare_msmarco/mrr/legend.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend entries={
\textsc{Eff-V-L-SPLADE~\cite{} (TC-quant)},
\textsc{Eff-V-L-SPLADE~\cite{} (DC-max)},
\textsc{DeepImpact~\cite{10.1145/3404835.3463030} (DC-max)},
\textsc{uniCOIL-Tilde~\cite{zhuang2021fast} (DC-max)},
\textsc{Eff-V-L-SPLADE~\cite{} (LS)},
\textsc{DeepImpact~\cite{10.1145/3404835.3463030} (LS)},
\textsc{uniCOIL-Tilde~\cite{zhuang2021fast} (LS)},
                        }]
         \addlegendimage{largespladeTplot};
         \addlegendimage{largespladeDplot};
         \addlegendimage{deepimpacDplot};
         \addlegendimage{unicoilDplot};
         \addlegendimage{largespladeVplot};
         \addlegendimage{deepimpacVplot};
         \addlegendimage{unicoilVplot};
        \end{customlegend}
\end{tikzpicture}


==> tikz/compare_msmarco/recall/figure.tex <==
\begin{figure}[ht]
     \centering
     \begin{subfigure}[h]{1.0\columnwidth}

     \begin{subfigure}[t]{\columnwidth}
         \centering
\adjustbox{max width=\textwidth}{%
%         \raisebox{50px}{%
         \input{tikz/compare_msmarco/recall/legend2.tex}}
%}
     \end{subfigure}

         \centering
\adjustbox{max width=\textwidth}{%
         \input{tikz/compare_msmarco/recall/pisa.tex}
         }
     
\adjustbox{max width=\textwidth}{%
         \input{tikz/compare_msmarco/mrr/pisa.tex}
         }
     \end{subfigure}
      
      \caption{Speedup vs Relative effectiveness comparison.}
     \label{fig:relative_effectiveness}
\end{figure}





==> tikz/compare_msmarco/recall/legend.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend columns=4,
legend entries={
\textsc{Eff-V-L-SPLADE~\cite{lassance2022efficiency} (T)},
\textsc{DeepImpact~\cite{deepimpactv1} (T)},
\textsc{uniCOIL-Tilde~\cite{tildetwo} (T)},
\textsc{BM25 (T)},
\textsc{Eff-V-L-SPLADE~\cite{lassance2022efficiency} (D)},
\textsc{DeepImpact~\cite{deepimpactv1} (D)},
\textsc{uniCOIL-Tilde~\cite{tildetwo} (D)},
\textsc{BM25 (D)},
\textsc{Eff-V-L-SPLADE~\cite{lassance2022efficiency} (A)},
\textsc{DeepImpact~\cite{deepimpactv1} (A)},
\textsc{uniCOIL-Tilde~\cite{tildetwo} (A)},
\textsc{BM25 (A)}
}]
         \addlegendimage{largespladeTplot};
         \addlegendimage{deepimpacTplot};
         \addlegendimage{unicoilTplot};
         \addlegendimage{bmvTplot};
         \addlegendimage{largespladeDplot};
         \addlegendimage{deepimpacDplot};
         \addlegendimage{unicoilDplot};
         \addlegendimage{bmvDplot};
         \addlegendimage{largespladeVplot};
         \addlegendimage{deepimpacVplot};
         \addlegendimage{unicoilVplot};
         \addlegendimage{bmvVplot};
        \end{customlegend}
\end{tikzpicture}


==> tikz/compare_msmarco/recall/legend2.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend columns=3,
legend entries={
\textsc{Eff-V-L-SPLADE (T)},
\textsc{Eff-V-L-SPLADE (D)},
\textsc{Eff-V-L-SPLADE (A)},
\textsc{DeepImpact (T)},
\textsc{DeepImpact (D)},
\textsc{DeepImpact (A)},
\textsc{uniCOIL-Tilde (T)},
\textsc{uniCOIL-Tilde (D)},
\textsc{uniCOIL-Tilde (A)},
\textsc{BM25 (T)},
\textsc{BM25 (D)},
\textsc{BM25 (A)}
}]
         \addlegendimage{largespladeTplot};
         \addlegendimage{largespladeDplot};
         \addlegendimage{largespladeVplot};
         \addlegendimage{deepimpacTplot};
         \addlegendimage{deepimpacDplot};
         \addlegendimage{deepimpacVplot};
         \addlegendimage{unicoilTplot};
         \addlegendimage{unicoilDplot};
         \addlegendimage{unicoilVplot};
         \addlegendimage{bmvTplot};
         \addlegendimage{bmvDplot};
         \addlegendimage{bmvVplot};
        \end{customlegend}
\end{tikzpicture}


==> tikz/compare_msmarco_indexsize/mrr/figure.tex <==
\begin{figure}[ht]
     \centering
     \begin{subfigure}[t]{0.7\columnwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{tikz/compare_msmarco/mrr/pisa.tex}
         }
     \end{subfigure}
     \begin{subfigure}[t]{0.29\columnwidth}
         \centering
\adjustbox{max width=\textwidth}{%
         \raisebox{50px}{%
         \input{tikz/compare_msmarco/mrr/legend.tex}}
}
     \end{subfigure}
      \caption{Speedup vs Relative MRR@10 comparison.}
     \label{fig:rq2}
\end{figure}





==> tikz/compare_msmarco_indexsize/mrr/legend.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend entries={
\textsc{Eff-V-L-SPLADE~\cite{} (TC-quant)},
\textsc{Eff-V-L-SPLADE~\cite{} (DC-max)},
\textsc{DeepImpact~\cite{10.1145/3404835.3463030} (DC-max)},
\textsc{uniCOIL-Tilde~\cite{zhuang2021fast} (DC-max)},
\textsc{Eff-V-L-SPLADE~\cite{} (LS)},
\textsc{DeepImpact~\cite{10.1145/3404835.3463030} (LS)},
\textsc{uniCOIL-Tilde~\cite{zhuang2021fast} (LS)},
                        }]
         \addlegendimage{largespladeTplot};
         \addlegendimage{largespladeDplot};
         \addlegendimage{deepimpacDplot};
         \addlegendimage{unicoilDplot};
         \addlegendimage{largespladeVplot};
         \addlegendimage{deepimpacVplot};
         \addlegendimage{unicoilVplot};
        \end{customlegend}
\end{tikzpicture}


==> tikz/compare_msmarco_indexsize/mrr/pisa.tex <==

   \begin{tikzpicture}
       \begin{axis}[
           xlabel=Speedup over unpruned, ylabel= Relative MRR@10,
           %title=MRR@10 comparison, title style={font=\huge},
           xmin=1.0, xmax=8.0, ymin=0.92, ymax=1.0,
           ]
         \addplot[largespladeTplot] table {tikz/compare_msmarco/mrr/splade_T.txt};
         \addplot[unicoilTplot] table {tikz/compare_msmarco/mrr/unicoil_T.txt};
         \addplot[deepimpacTplot] table {tikz/compare_msmarco/mrr/deep_impact_T.txt};
         \addplot[bmvTplot] table {tikz/compare_msmarco/mrr/bm25_T.txt};
         \addplot[largespladeDplot] table {tikz/compare_msmarco/mrr/splade_D.txt};
         \addplot[deepimpacDplot] table {tikz/compare_msmarco/mrr/deep_impact_D.txt};
         \addplot[unicoilDplot] table {tikz/compare_msmarco/mrr/unicoil_D.txt};
         \addplot[bmvDplot] table {tikz/compare_msmarco/mrr/bm25_D.txt};
         \addplot[largespladeVplot] table {tikz/compare_msmarco/mrr/splade_V.txt};
         \addplot[deepimpacVplot] table {tikz/compare_msmarco/mrr/deep_impact_V.txt};
         \addplot[unicoilVplot] table {tikz/compare_msmarco/mrr/unicoil_V.txt};
         \addplot[bmvVplot] table {tikz/compare_msmarco/mrr/bm25_V.txt};
%         \draw[very thick, olive] (2,0.98) rectangle (8,1.0);
%         \draw[very thick, red] (4,0.92) rectangle (8,0.98);
         \fill[nearly transparent, olive] (2,0.98) rectangle (8,1.0);
         \fill[very nearly transparent, red] (4,0.92) rectangle (8,0.98);
       \end{axis}
    \end{tikzpicture}


==> tikz/compare_msmarco_indexsize/recall/figure.tex <==
\begin{figure}[ht]
     \centering
     \begin{subfigure}[h]{1.0\columnwidth}

     \begin{subfigure}[t]{\columnwidth}
         \centering
\adjustbox{max width=\textwidth}{%
%         \raisebox{50px}{%
         \input{tikz/compare_msmarco/recall/legend2.tex}}
%}
     \end{subfigure}

         \centering
\adjustbox{max width=\textwidth}{%
         \input{tikz/compare_msmarco/recall/pisa.tex}
         }
     
\adjustbox{max width=\textwidth}{%
         \input{tikz/compare_msmarco/mrr/pisa.tex}
         }
     \end{subfigure}
      
      \caption{Speedup vs Relative effectiveness comparison.}
     \label{fig:relative_effectiveness}
\end{figure}





==> tikz/compare_msmarco_indexsize/recall/figure2.tex <==
\begin{figure*}[ht]
     \centering
     \begin{subfigure}[hy]{0.85\columnwidth}
     \adjustbox{max width=\textwidth}{%
         \input{tikz/compare_msmarco/recall/pisa.tex}
     }
     \end{subfigure}
     \begin{subfigure}[ht]{0.3\columnwidth}
     \adjustbox{max width=\textwidth}{%
         \input{tikz/compare_msmarco/recall/legend3.tex}
     }
     \end{subfigure}
     \begin{subfigure}[ht]{0.85\columnwidth}
     \adjustbox{max width=\textwidth}{%
         \input{tikz/compare_msmarco/mrr/pisa.tex}
     }
     \end{subfigure}
      
      \caption{Speedup vs relative effectiveness comparison. Rectangles show the two desired conditions (Green $\geq 2\times$ speedup with $\leq 2\%$ effectiveness drop, Red $\geq 4\times$ speedup with $\leq 8\%$ effectiveness drop).}
     \label{fig:relative_effectiveness}
\end{figure*}





==> tikz/compare_msmarco_indexsize/recall/legend.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend columns=4,
legend entries={
\textsc{Eff-V-L-SPLADE~\cite{lassance2022efficiency} (T)},
\textsc{DeepImpact~\cite{deepimpactv1} (T)},
\textsc{uniCOIL-Tilde~\cite{tildetwo} (T)},
\textsc{BM25 (T)},
\textsc{Eff-V-L-SPLADE~\cite{lassance2022efficiency} (D)},
\textsc{DeepImpact~\cite{deepimpactv1} (D)},
\textsc{uniCOIL-Tilde~\cite{tildetwo} (D)},
\textsc{BM25 (D)},
\textsc{Eff-V-L-SPLADE~\cite{lassance2022efficiency} (A)},
\textsc{DeepImpact~\cite{deepimpactv1} (A)},
\textsc{uniCOIL-Tilde~\cite{tildetwo} (A)},
\textsc{BM25 (A)}
}]
         \addlegendimage{largespladeTplot};
         \addlegendimage{deepimpacTplot};
         \addlegendimage{unicoilTplot};
         \addlegendimage{bmvTplot};
         \addlegendimage{largespladeDplot};
         \addlegendimage{deepimpacDplot};
         \addlegendimage{unicoilDplot};
         \addlegendimage{bmvDplot};
         \addlegendimage{largespladeVplot};
         \addlegendimage{deepimpacVplot};
         \addlegendimage{unicoilVplot};
         \addlegendimage{bmvVplot};
        \end{customlegend}
\end{tikzpicture}


==> tikz/compare_msmarco_indexsize/recall/legend2.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend columns=3,
legend entries={
\textsc{Eff-V-L-SPLADE (T)},
\textsc{Eff-V-L-SPLADE (D)},
\textsc{Eff-V-L-SPLADE (A)},
\textsc{DeepImpact (T)},
\textsc{DeepImpact (D)},
\textsc{DeepImpact (A)},
\textsc{uniCOIL-Tilde (T)},
\textsc{uniCOIL-Tilde (D)},
\textsc{uniCOIL-Tilde (A)},
\textsc{BM25 (T)},
\textsc{BM25 (D)},
\textsc{BM25 (A)}
}]
         \addlegendimage{largespladeTplot};
         \addlegendimage{largespladeDplot};
         \addlegendimage{largespladeVplot};
         \addlegendimage{deepimpacTplot};
         \addlegendimage{deepimpacDplot};
         \addlegendimage{deepimpacVplot};
         \addlegendimage{unicoilTplot};
         \addlegendimage{unicoilDplot};
         \addlegendimage{unicoilVplot};
         \addlegendimage{bmvTplot};
         \addlegendimage{bmvDplot};
         \addlegendimage{bmvVplot};
        \end{customlegend}
\end{tikzpicture}


==> tikz/compare_msmarco_indexsize/recall/legend3.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend columns=1,
legend entries={
\textsc{Eff-V-L-SPLADE (T)},
\textsc{Eff-V-L-SPLADE (D)},
\textsc{Eff-V-L-SPLADE (A)},
\textsc{DeepImpact (T)},
\textsc{DeepImpact (D)},
\textsc{DeepImpact (A)},
\textsc{uniCOIL-Tilde (T)},
\textsc{uniCOIL-Tilde (D)},
\textsc{uniCOIL-Tilde (A)},
\textsc{BM25 (T)},
\textsc{BM25 (D)},
\textsc{BM25 (A)}
}]
         \addlegendimage{largespladeTplot};
         \addlegendimage{largespladeDplot};
         \addlegendimage{largespladeVplot};
         \addlegendimage{deepimpacTplot};
         \addlegendimage{deepimpacDplot};
         \addlegendimage{deepimpacVplot};
         \addlegendimage{unicoilTplot};
         \addlegendimage{unicoilDplot};
         \addlegendimage{unicoilVplot};
         \addlegendimage{bmvTplot};
         \addlegendimage{bmvDplot};
         \addlegendimage{bmvVplot};
        \end{customlegend}
\end{tikzpicture}


==> tikz/compare_msmarco_indexsize/recall/pisa.tex <==
   \begin{tikzpicture}
       \begin{axis}[
           xlabel=Speedup over unpruned, ylabel= Relative Recall@1k,
           %title=Recall@1k comparison, title style={font=\huge},
           xmin=1.0, xmax=8.0, ymin=0.92, ymax=1.0,
           ]
         \addplot[largespladeTplot] table {tikz/compare_msmarco/recall/splade_T.txt};
         \addplot[unicoilTplot] table {tikz/compare_msmarco/recall/unicoil_T.txt};
         \addplot[deepimpacTplot] table {tikz/compare_msmarco/recall/deep_impact_T.txt};
         \addplot[bmvTplot] table {tikz/compare_msmarco/recall/bm25_T.txt};
         \addplot[largespladeDplot] table {tikz/compare_msmarco/recall/splade_D.txt};
         \addplot[deepimpacDplot] table {tikz/compare_msmarco/recall/deep_impact_D.txt};
         \addplot[unicoilDplot] table {tikz/compare_msmarco/recall/unicoil_D.txt};
         \addplot[bmvDplot] table {tikz/compare_msmarco/recall/bm25_D.txt};
         \addplot[largespladeVplot] table {tikz/compare_msmarco/recall/splade_V.txt};
         \addplot[deepimpacVplot] table {tikz/compare_msmarco/recall/deep_impact_V.txt};
         \addplot[unicoilVplot] table {tikz/compare_msmarco/recall/unicoil_V.txt};
         \addplot[bmvVplot] table {tikz/compare_msmarco/recall/bm25_V.txt};

%         \draw[very thick, olive] (2,0.98) rectangle (8,1.0);
%         \draw[very thick, red] (4,0.92) rectangle (8,0.98);
         \fill[nearly transparent, olive] (2,0.98) rectangle (8,1.0);
         \fill[very nearly transparent, red] (4,0.92) rectangle (8,0.98);
         
       \end{axis}
    \end{tikzpicture}

